Deja Vu: Contextual Sparsity for Efficient LLMs at Inference Time

Large language models (LLMs) with hundreds of billions of parameters have sparked a new wave of exciting AI applications. However, they are computationally expensive at inference time. Sparsity is a natural approach to reduce this cost, but existing methods either require costly retraining, have to forgo LLM's in-context learning ability, or do not yield wall-clock time speedup on modern hardware. We hypothesize that contextual sparsity, which are small, input-dependent sets of attention heads and MLP parameters that yield approximately the same output as the dense model for a given input, can address these issues. We show that contextual sparsity exists, that it can be accurately predicted, and that we can exploit it to speed up LLM inference in wall-clock time without compromising LLM's quality or in-context learning ability. Based on these insights, we propose DejaVu, a system that uses a low-cost algorithm to predict contextual sparsity on the fly given inputs to each layer, along with an asynchronous and hardware-aware implementation that speeds up LLM inference. We validate that DejaVu can reduce the inference latency of OPT-175B by over 2X compared to the state-of-the-art FasterTransformer, and over 6X compared to the widely used Hugging Face implementation, without compromising model quality. The code is available at https://github.com/FMInference/DejaVu.

==> icml2022/trash.tex <==


\iffalse
\begin{lemma}
A better bound 
\begin{align*}
(1-\epsilon) \cdot \| x \|_2 \leq \| f(x) \|_2 \leq (1+\epsilon) \cdot \| x \|_2
\end{align*}
\end{lemma}

What assumptions are we allowed to make
\begin{itemize}
    \item $W$,
    \item $K$
    \item $V$
    \item In practice, for big model $d = 10^4$ vs $s < 2000$, this means $d \geq s$
\end{itemize}
Where do we use ReLU?
\fi


\iffalse
\begin{definition}[Approximate Nearest Neighbor ($\ann$)]\label{def:app_nearest_neighbor}
Let $\ov{c} >1$ and $r \in (0,2)$ denote two parameters.  Given an $n$-vector set $Y \subset \mathbb{S}^{d-1}$ on a unit sphere, the objective of the $(\ov{c},r)$-Approximate Nearest Neighbor ($\ann$) is to construct a data structure that, for any query $x \in \mathbb{S}^{d-1}$ such that $\min_{y\in Y}\| y - x \|_2 \leq r$, it returns a vector $z$ from $Y$ that satisfies $\| z - x \|_2 \leq \ov{c} \cdot r$.
\end{definition}

In the iterative-type optimization algorithm, the cost per iteration could be dominated by the Approximate $\maxip$ problem (Definition~\ref{def:app_maxip}), which is the dual problem of the $(\ov{c},r)$-$\ann$.

\begin{definition}[Approximate $\maxip$]\label{def:app_maxip}
Let $c \in (0,1)$ and $\tau \in (0,1)$ denote two parameters.
Given an $n$-vector dataset $Y \subset \mathbb{S}^{d-1}$ on a unit sphere, the objective of the $(c,\tau)$-{$\maxip$} is to construct a data structure that, given a query $x \in \mathbb{S}^{d-1}$ such that $\max_{y\in Y}\langle x , y \rangle \geq \tau$, it retrieves a vector $z$ from $Y$ that satisfies $\langle x , z \rangle \geq c \cdot \max_{y \in Y} \langle x,y \rangle$.
\end{definition}

Next, we present the the primal-dual connection between $\ann$ and approximate $\maxip$. Given to unit vectors $x,y\in \R^d$ with both norm equal to $1$, $\|x-y\|_2^2 = 2 - 2\langle x , y \rangle$. Therefore, we could maximizing  $\langle x , y \rangle$ by minimizing $\|x-y\|_2^2$. Based on this connection, we present how to solve $(c,\tau)$-{$\maxip$} using $(\ov{c},r)$-{$\ann$}.  We start with showing how to solve $(\ov{c},r)$-{$\ann$} with {\lsh}.


\begin{theorem}[Andoni, Laarhoven, Razenshteyn and Waingarten~\cite{alrw17}]\label{thm:alrw17}
Let $\ov{c} > 1$ and $r \in (0,2)$ denote two parameters. One can solve $(\ov{c},r)$-$\ann$ on a unit sphere in query time $O(d \cdot n^{\rho})$ using preprocessing time $O(dn^{1+o(1)})$ and space $O(n^{1+o(1)} + d n)$, where $\rho = \frac{2}{\ov{c}^2} -\frac{1}{\ov{c}^4}+o(1)$.
\end{theorem}

Next, we solve $(c,\tau)$-{$\maxip$} by solving  $(\ov{c},r)$-{$\ann$} using Theorem~\ref{thm:alrw17}. We have 

\begin{corollary}[An informal statement of Corollary~\ref{coro:maxip_lsh_formal}]\label{coro:maxip_lsh_informal}
Let $c \in (0,1)$ and $\tau \in (0,1)$ denote two parameters. One can solve $(c,\tau)$-{$\maxip$} on a unit sphere $\mathcal{S}^{d-1}$ in query time $O(d \cdot n^{\rho})$, where $\rho\in(0,1)$, using {\lsh} with both preprocessing time and space in $O(d n^{1+o(1)})$.
\end{corollary}

In our work, we consider a generalized form of approximate $\maxip$, denoted as projected approximate $\maxip$.

\begin{definition}[Projected approximate $\maxip$]\label{def:proj_approximate_maxip_informal}
Let $\phi, \psi: \R^d \rightarrow \R^k$ denote two transforms. Given an $n$-vector dataset $Y \subset \R^d $ so that $\psi(Y) \subset \mathbb{S}^{k-1}$, the goal of the $(c,\phi, \psi,\tau)$-{$\maxip$} is to construct a data structure that, given a query $x\in \R^d$ and $\phi(x) \in \mathbb{S}^{k-1}$ such that $\max_{y\in Y}\langle \phi(x) , \psi(y) \rangle \geq \tau$, it retrieves a vector $z \in Y$ that satisfies $\langle \phi(x) , \psi(z) \rangle \geq c \cdot (\phi, \psi)\text{-}\maxip (x,Y)$.
\end{definition}

For details of space-time trade-offs, please refer to Section~\ref{sec:data_structure}. The following sections show how to use projected approximate $\maxip$ to accelerate the optimization algorithm by reducing the cost per iteration.
\fi

\iffalse
\begin{definition}[Regularized $\minip$]\label{def:reg_minip} 
Given a data set $Y\subseteq \R^d$ and a point $x\in\R^d$. Let $\phi:\R^d\rightarrow \R^d$ denote a mapping. Given a constant $\alpha$, we define regularized $\minip$ as follows:
\begin{align*}
    (\phi,\alpha)\text{-}\minip (x,Y) := \min_{y \in Y} \langle y-x,\phi(x) \rangle + \alpha\|x-y\|.
\end{align*}
\end{definition}
\fi




\iffalse
\Zhao{I don't think we need the following things}
\subsection{Definitions and  Properties for Optimization}

We start with listing definitions for optimization.
\begin{definition}[Convex hull and its diameter]\label{def:cvx_hull}
Given a set $A=\{x_i\}_{i\in [n]} \subset \R^d$, we define its convex hull $\mathcal{B}(A)$ to be the collection of all finite linear combinations $y$ that satisfies  $ y=\sum_{i\in [n]} a_i\cdot x_i$ where $a_i\in [0,1]$ for all $i\in[n]$ and $\sum_{i\in [n]}a_i= 1$.  Let $D_{\max}$ denote the maximum square of diameter of ${\cal B}(A)$ so that $\|x-y\|_2\leq D_{\max}$ for all $(x,y)\in {\cal B}(A)$.
\end{definition}




\begin{definition}[Smoothness]\label{def:smooth}
We say $L$ is $\beta$-smooth if 
\begin{align*}
L(y)\leq L(x)+\langle \nabla L(x),y-x \rangle+\frac{\beta}{2}\| y-x \|^2_2
\end{align*}
\end{definition}



\begin{definition}[Convex]\label{def:convex}
We say function $L$ is convex if 
\begin{align*}
L(x)\geq L(y)+\langle \nabla L(y),x-y \rangle
\end{align*}
\end{definition}



Next, we list properties for optimization.
\begin{corollary}\label{coro:hull_maxip}
For a set $A=\{x_i\}_{i\in [n]} \subset \R^d$, and its convex hull $\mathcal{B}(A)$, given a query $q\in \R^d$, if $x^*=\arg\max_{x\in A} q^\top x$. Then, $q^\top y \leq q^\top x^*$ for all $y\in \mathcal{B}(A)$.
\end{corollary}
\begin{proof}
We can upper bound $q^\top y$ as follows:
\begin{align*}
    q^\top y 
    =&~q^\top (\sum_{i\in [n]}a_i\cdot x_i)  \\
    = &~ \sum_{i\in [n]}a_i\cdot q^\top x_i\\
    \leq &~ \sum_{i\in [n]}a_i\cdot q^\top x^*\\
    \leq &~ q^\top x^*
\end{align*}
where the first step follows from the definition of convex hull in Definition~\ref{def:cvx_hull}, the second step is an reorganization, the third step follows the fact that $a_i\in [0,1]$ for all $i\in[n]$ and $q^\top x_i \leq q^\top x^*$ for all $x_i\in A$, the last step follows that $\sum_{i\in [n]}a_i= 1$.
\end{proof}




\begin{lemma}[$\maxip$ condition] \label{lemma:max_ip_condition}
Let $g : \R^d \rightarrow \R$ denote a convex function. Let $S \subset \R^d$ denote a set of points. Given a vector $x\in {\cal B}(S)$, we have
\begin{align*}
\min_{s \in S } \langle \nabla g(x) ,  s-x \rangle  \leq 0, ~~~ \forall x\in \cal{B}(S).
\end{align*}
\end{lemma}

\begin{proof}
Let $s_{\min}=\arg\min_{s\in S} \langle \nabla g(x) ,  s \rangle $. Then, we upper bound $\langle \nabla g(x) ,  s_{\min}-x \rangle$ as
\begin{align}\label{eq:maxip_s_0}
    \langle \nabla g(x) ,  s_{\min}-x \rangle =&~\langle \nabla g(x) ,  s_{\min}-\sum_{s\in S} a_i\cdot s \rangle\notag\\
    \leq &~\langle \nabla g(x) ,  \sum_{s\in S}a_i( s_{\min}- s_i) \rangle \notag\\
    = &~\sum_{s_i\in S}a_i \langle \nabla g(x) ,   s_{\min}- s_i \rangle \notag\\
    = &~\sum_{s_i\in S}a_i (\langle \nabla g(x) ,   s_{\min} \rangle -\langle \nabla g(x) ,   s_i \rangle )\notag\\
    \leq&~ 0
\end{align}
where the first step follows from the definition of convex hull in Definition~\ref{def:cvx_hull}, the second and third steps are reorganizations, the final steps follows that $\langle \nabla g(x) ,   s_0 \rangle \leq \langle \nabla g(x) ,   s \rangle$ for all $s\in S$.

Next, we upper bound $\min_{s \in S } \langle \nabla g(x) ,  s-x \rangle  \leq 0, ~~~ \forall x\in \cal{B}(S)$ as
\begin{align*}
    \min_{s \in S } \langle \nabla g(x) ,  s-x \rangle  \leq  \langle \nabla g(x) ,  s_0-x \rangle  \leq 0
\end{align*}
where the first step follows from the definition of function $\min$ and the second step follows from Eq~\eqref{eq:maxip_s_0}.
\end{proof}
\fi 
